That Was Then, This Is Now: A Security Evaluation of Password Generation, Storage, and Autofill in Thirteen Password Managers

Password managers have the potential to help users more effectively manage their passwords and address many of the concerns surrounding password-based authentication, however prior research has identified significant vulnerabilities in existing password managers. Since that time, five years has passed, leaving it unclear whether password managers remain vulnerable or whether they are now ready for broad adoption. To answer this question, we evaluate thirteen popular password managers and consider all three stages of the password manager lifecycle--password generation, storage, and autofill. Our evaluation is the first analysis of password generation in password managers, finding several non-random character distributions and identifying instances where generated passwords were vulnerable to online and offline guessing attacks. For password storage and autofill, we replicate past evaluations, demonstrating that while password managers have improved in the half-decade since those prior evaluations, there are still significant issues, particularly with browser-based password managers; these problems include unencrypted metadata, unsafe defaults, and vulnerabilities to clickjacking attacks. Based on our results, we identify password managers to avoid, provide recommendations on how to improve existing password managers, and identify areas of future research.

==> extras.tex <==
\subsection{Removed Analysis}
One of the most clear differences between the password generators was that the symbol set size varied widely. As can be seen in Table~\ref{tab:symbolset} Chrome, RoboForm, LastPass and Bitwarden had 8 or less available symbols, while the next smallest symbol set was 20 symbols. As can be seen in Figure~\ref{fig:informationentropy} and Figure~\ref{fig:shannonentropyall}, this change in symbol set size reduces both information entropy and Shannon entropy. While some password managers might be trying to avoid SQL injection attacks or other attacks that rely on certain symbols by reducing the symbol set, NIST has noted such precautions are unnecessary if the password is properly hashed~\footnote{\url{https://pages.nist.gov/800-63-3/sp800-63b/appA_memorized.html}}. There is therefore no reason not to use the maximum number of characters possible to increase entropy. 

Florenicio~\cite{florencio2014administrator} estimated that to resist online attacks a password must require $10^6$ guesses to crack and to resist offline attacks it must require $10^{14}$ guesses to crack. The average number of guesses required to brute force a password is calculated by taking the number of possible combinations ($2^{number_bits}$) and dividing by two. That means to resist an online attack you would need at least 21 bits of entropy because $\frac{(2^{21})}{2} = 1048576$ and provides the needed $10^6$ guesses. Likewise, to resist an offline attack would require 48 bits of entropy to provide $10^{14}$ guesses. Figure~\ref{fig:informationentropy} shows that even for passwords of only length 8, all password managers surveyed provide enough entropy to resist online attacks. Other than Chrome and RoboForm all other password managers appear to provide sufficient entropy to resist offline attacks, but LastPass and Bitwarden are barely over the minium required entropy. 

\begin{figure}
	\includegraphics[width=\columnwidth]{Images/genstats/info_entropy/information_entropy_bar_8_mod.png}
	\caption{Information Entropy Ordered by Character Set Size}
	\label{fig:informationentropy}
\end{figure}



\subsection{Other remove analysis}

Browser-based password managers have a lot of catching up to do. They have less features and are protected by system level or application level accounts rather than a Master Password specific to the password manager. Browsers enable password management by default. However, given that they lack protection via a Master Password and other common features, it would be better if they prompted the user to enable this feature when first installing the browser rather than enabling it by default. The user might accidentally click on the 'save password' popup and save credentials unintentionally. Of the browser-based password managers surveyd, Safari was the most secure in our estimation because it disallowed autofill and provides password generation via iCloud Keychain. 

Of the extension-based and standalone password managers, 1Password has the strongest default security posture in our estimation, avoiding the pitfalls of autofill by requiring user interaction, using a decent symbol set size for password generation and securing stored passwords appropriately. In contrast, LastPass preferred convenience over security in its default settings, allowing autofill by default in spite of known vulernabilities and requiring no pin by default for its authenticator app. These default settings can be changed in LastPass, but why not prefer a more secure stance from the start? Bitwarden takes this approach, requiring a user to enable autofill and providing a clear warning that this feature is insecure. 

KeePassXC stood out in that it properly cleared the clipboard after a password was copied, but it lacked true multifactor authentication. Some users might appreciate that their database is only stored locally rather than being backed up in the cloud if they are concerned with privacy. But there is a downside to this approach if the local copy is ever lost or compromised. Below are some more specific suggestions for improvement and observations about individual password managers. 

\subsection{LastPass Authenticator App}

LastPass has its own one time password app and allows users to use its own authenticator app for multifactor authentication. All other password managers that provide one time passwords discourage or disallow using their own authenticator for their service. LastPass should follow suit. 1Password compares this practice to locking your car keys in the car because you have to login to 1Password to access the credential you want to use to login to 1Password. While LastPass does not suffer from this same problem, since the authenticator app uses separate login credentials, using an authenticator app from your password manager is like hiring a locksmith from the same company that installs your security system for your house. Yes, you can do it. But shouldn't you diversify your security portfolio a bit?

\subsection{LastPass One-Time Password Vulnerability Patched}\label{sub:lpasspatch}

In 2014, Li~\cite{li2014emperor} observed that one-time password generation in LastPass was vulnerable due to the lack of a CSRF token. Because LastPass did not know the OTP or the master key, it could not validate \path{rand_encrypted_key}. The adversary, Mallory, could therefore fetch Alice's encrypted password database via the OTP page. Mallory could then proceed to perform an offline guessing attack or perform a denial of service attack by deleting encrypted values. Figure~\ref{fig:otpfix} shows that this vulnerability was fixed via the addition of a CSRF token. 

\begin{figure*}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/8_zxcvbn_std_scatter.png}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/12_zxcvbn_std_scatter.png}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/20_zxcvbn_std_scatter.png}
    \caption{Standard Deviation for zxcvbn Guess Estimates}
    \captionsetup{aboveskip=0pt,font=it}
    \caption*{\\The mean for each length in log10(number guesses) was approximately 8, 12 and 20 respectively}
    \label{fig:zxcvbnstddev}
\end{figure*}

\begin{figure*}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/8_zxcvbn_mean_scatter.png}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/12_zxcvbn_mean_scatter.png}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/20_zxcvbn_mean_scatter.png}
    \caption{zxcvbn Mean Number of Guesses}
    \label{fig:zxcvbnmean}
\end{figure*}

\begin{figure*}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/8_zxcvbn_std_scatter.png}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/12_zxcvbn_std_scatter.png}
    \includegraphics[width=.33\textwidth]{Images/zxcvbn/20_zxcvbn_std_scatter.png}
    \caption{zxcvbn Standard Deviation}
    \label{fig:zxcvbnstddev}
\end{figure*}

\begin{figure}
    \includegraphics[width=\columnwidth]{Images/autofill/otp_fix.png}
    \caption{LastPass One-Time Password Vulnerability Fixed via CSRF Token}
    \label{fig:otpfix}
\end{figure}


\begin{figure}[h]
    \includegraphics[scale=.5]{Images/genstats/numchars_scatter.png}
    \caption{Character Set Sizes}
    \label{fig:charactersetsize}
\end{figure}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lG@{}}
    \\ \midrule
    \rowcolor{white}
    \textbf{8lpassall}       & \verb|$*!@^#&%uHqMgiCtxKzrNoaDJpSkIbYZUcXAyhmGfREdLBVWewvsTlQOnFPj5712380649| \\
    \rowcolor{white}
    \textbf{12lpassall}       & \verb|*@$&!#%^dEJHjZQAOgkyafnlBLVYFoDmsSvpwICPXxRUqMezWthTKcuNGrbi6514203987| \\
    \rowcolor{white}
    \textbf{20lpassall}       & \verb|%$&!#@*^jAtlYRNfOKzywQbGPWhMiTUgnoDqJVSHecsmBdrIxaZpEuXkFvLC9318245067| \\
    \textbf{8lpassl}       & \verb|uEJFcSVhfLKIUplYjQnoRzyvsGgWaNkwZPqeDiTMrXAdBObCHtmx| \\
    \textbf{12lpassl}       & \verb|JmUOWeGBxMTqglRNakCHVXbrozpwndsyDiEAtjchZSuFKILvYQfP| \\
    \textbf{20lpassl}       & \verb|FbEKnkCAWdejHfXhVSRqmUDrctuaysgiOPvlGTMpJzoBQYIZwLNx| \\
    \rowcolor{white}
    \textbf{8lpassld}       & \verb|cskKvywuAYbGgInWTpRxDQPCzhZNUteELJBdXifVHjmqSMaFrloO3710849625| \\
    \rowcolor{white}
    \textbf{12lpassld}       & \verb|korOCJEdxQqeIwtUNhTDRuvansjimbMHyPKLZFzBWAfGXSYlgpcV7209143865| \\
    \rowcolor{white}
    \textbf{20lpassld}       & \verb|iplBnhumsLKtSJfIHTORMGXwaQNzrPkgdEeUybojCFxYZqcWvVDA6078392154| \\
    \textbf{8lpassls}       & \verb|%&$*^#@!yzHRBulQSigJoEfKtrNqApheZwWdjTbLnFOvaCcDVXMmPskYUIGx| \\
    \textbf{12lpassls}       & \verb|!@#^%&*$WBvaOQfAJzSXrhDZRGuLVPoidkUbNsmTCYgqFjptKnElIyweHMcx| \\
    \textbf{20lpassls}       & \verb|%&*@#$!^WkerdQEhZcYbjxzsVHATUPJgRinFqXCGpwSMyoamDIOBlNuKtvLf| \\
    \rowcolor{white}
    \textbf{8lpasssd}       & \verb|@!#^%*$&7430286195| \\
    \rowcolor{white}
    \textbf{12lpasssd}       & \verb|^#!*@$&%1403852769| \\
    \rowcolor{white}
    \textbf{20lpasssd}       & \verb|@%*^#&!$6582013947| \\
    \\ \bottomrule
    \end{tabular}
    \caption{LastPass Password Generation: Characters Sorted by Frequency}
    \captionsetup{aboveskip=0pt,font=it}
    \label{tab:lpasscharfreq}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lG@{}}
    \\ \midrule
    \rowcolor{white}
    \textbf{8onepsall}       & \verb|1486075923=~%-_?#).>+@!]:}*^,MwpCcUjQWsfkDabFTVzKhXgPEAZvGouYritNBJmeqRHLynxd| \\
    \rowcolor{white}
    \textbf{12onepsall}       & \verb|9537168402.-]~,^)@:>=#!*+_?}%iuYMrVJfXpsNLqkbTvtWyRPjUCzHBxKAnemZwDGhoFEQgcad| \\
    \rowcolor{white}
    \textbf{20onepsall}       & \verb|9613057842>*^:-=%?@+.}~,#]!_)dVuDbaZNCJRTYAEoKrgnUGijtxkysBHQewLqvczWMFmPXfph| \\
    \textbf{8onepsl}       & \verb|tEfqXjFHNrpKmnayBxQcgVsAJiMdUbwLhkCZzRTPWYGDevuo| \\
    \textbf{12onepsl}       & \verb|DvQBkNVGoJzhryTuAbFEgsYwxdcMUitHqPCfLWpeKRnaZmjX| \\
    \textbf{20onepsl}       & \verb|JvNbZpsdgkUCzQiKHrfADXYyFLctGjueEVxTMaowhRmWBPqn| \\
    \rowcolor{white}
    \textbf{8onepsld}       & \verb|4095683721ePLFXTsaqGiVjmCUEnMbthRfYBNvyKZczpDgrHQkJuAoxdwW| \\
    \rowcolor{white}
    \textbf{12onepsld}       & \verb|1304286957WEHxJnrZKPRLFsXeiqMAYgpTjbtdyBhGuUcDNwmCzkvafVoQ| \\
    \rowcolor{white}
    \textbf{20onepsld}       & \verb|4895263701xahXyDjefmQWAorNHGLPdwpnFsJYuUZzvBqbViTtcgMKCkER| \\
    \textbf{8onepsls}       & \verb|>~!^*_)#+@-%.}],:?=QKmFAXaEbwZhgWzvxUVpktcTdfBjDGCMPeqrsHnyouNYLRJi| \\
    \textbf{12onepsls}       & \verb|~=#%-*@}_]!^),.:>+?rbGCgdjzhHyRXYoDmWxqiMPVunQNUpBZwvFfkeJTtELsacKA| \\
    \textbf{20onepsls}       & \verb|?%b+@:}#,y!Ev.h^j=*qMZ-HawxQDz)g]~sdGepiWc>rTmARKktCVBJFuoUX_NnYLPf| \\
    \\ \bottomrule
    \end{tabular}
    \caption{1Password Password Generation: Characters Sorted by Frequency}
    \captionsetup{aboveskip=0pt,font=it}
    \label{tab:1passcharfreq}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lG@{}}
    \\ \midrule
    \rowcolor{white}
    \textbf{8roboall}       & \verb|%!^@$#4627583NPHFDJUXACTSGMERBKLQVYWqmgasneokfvptbuhyixdwrcjzZ9| \\
    \rowcolor{white}
    \textbf{12roboall}       & \verb|$%#^!@2637548BHGFSQECXWYJRDNMUALVPTKdtboenhskjvqaicgwpmxfyur9zZ| \\
    \rowcolor{white}
    \textbf{20roboall}       & \verb|%#@!^$8462735XHVPJWCUFKLYNDESAMTQRiBGgdveaspnkytqjfbmxwrcuoh9Zz| \\
    \textbf{8robol}       & \verb|GHDYEQKPJFURCTASNLVMXBWpyikuvmtofxecasdwjngbhqrZ| \\
    \textbf{12robol}       & \verb|VMDFQAGNRLUEXKCJSBPWTYHcmfiqyawnektsdvrgjhopxbuZ| \\
    \textbf{20robol}       & \verb|REFQWJUTBKDGCMAHSVPXYLNfkvyjsnhwoepabqixgdturcmZ| \\
    \rowcolor{white}
    \textbf{8robold}       & \verb|5782346RUALJDQFHSPKEVGTMYBXCNWhynabrqwpkfumxjvctodsigeZ9| \\
    \rowcolor{white}
    \textbf{12robold}       & \verb|6853247JUWYSBLTQFGCRMPVKANXHEDgcidbjtwpesafxqvhmrkounyZ9| \\
    \rowcolor{white}
    \textbf{20robold}       & \verb|6532874MTJFSVCYDNHPLGWEXQABUnRkeKswpjughytdqbircafovxm9Z| \\
    \textbf{8robols}       & \verb|%@^$#!SLFWVAURKNTEXDQJYBMHPGCavhtndwcjkyufxieqobrgpmszZ| \\
    \textbf{12robols}       & \verb|$^%#@!FHJVESBGMUYXDLTPCAQNWRKrwogjhicexmsyftvkqdabupnZz| \\
    \textbf{20robols}       & \verb|%@$^#!PFAXTKBQCSHDGVJEMWRYtNgUfLabyshrkpwmdouvqxjineczZ| \\
    \rowcolor{white}
    \textbf{8robosd}       & \verb|#$@%!^65324879| \\
    \rowcolor{white}
    \textbf{12robosd}       & \verb|$@!#^%57263489| \\
    \rowcolor{white}
    \textbf{20robosd}       & \verb|@^!$#%63582749| \\
    \\ \bottomrule
    \end{tabular}
    \caption{RoboForm Password Generation: Characters Sorted by Frequency}
    \captionsetup{aboveskip=0pt,font=it}
    \label{tab:robocharfreq}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lG@{}}
    \\ \midrule
    \rowcolor{white}
    \textbf{8dlanall}       & \verb|7849536PMLJSRCAEHNFKBXGYQTDphbnmfrzoqcsygxetdkaij($".*=_||\verb|{]!;[~</,%)>`@'#:&?-+}\^| \\
    \rowcolor{white}
    \textbf{12dlanall}       & \verb|3498576QNBHPAFMXJCYKTGSDRLEdqzmnpsfjghbtxckaioyre/$#{!<-,?"(\=].~*^'+`||\verb|:;}>_)[%@&| \\
    \rowcolor{white}
    \textbf{20dlanall}       & \verb|5763948QPRDHAFSNMKYLTBCXGEJipjengtryfhscbadqxkmz~*@_'={)[,.#&:!;$+/(-"||\verb|%^}]?o`><\wuU2WvVZ| \\
    \textbf{8dlanl}       & \verb|HNCXJBFYSQPKAGLTREMDqjbsozemrkxfgtycandihp| \\
    \textbf{12dlanl}       & \verb|FKJMTRXAGSQCPENLHDBYkmjgqofpazenbdrtchsixy| \\
    \textbf{20dlanl}       & \verb|MXHQEDNTFLCGJBKYPRSAbjhtpqzndkaixyemscgfrouVwvWZU| \\
    \rowcolor{white}
    \textbf{8dlanld}       & \verb|9457368HEDNTCSRPKFBGQJXAMYLaoqjkibgmrtcsnxdhpyfze| \\
    \rowcolor{white}
    \textbf{12dlanld}       & \verb|6859743AQEKGSBFPTJCDLXRHNYMkbxqmnztdoaehfsicpjyrg| \\
    \rowcolor{white}
    \textbf{20dlanld}       & \verb|4573689YNGMEXBDJLFCSHARQPKThjqacigrkpynmbzsfdetxouVZWUw2v| \\
    \textbf{8dlanls}       & \verb|PRSEJQGFLKNAMYDTHXBCjzgbhtcdfqypneorikxmas"!?$#%*^\<@;||\verb|~]>-'_,/:.&[`{=+)(}| \\
    \textbf{12dlanls}       & \verb|YTXPRCQJMNBFAHLESGKDketfgpozbmynidrxasjhqc["=$)}:*(+<!'?>@`&#._^||\verb|~-;,\]{/%| \\
    \textbf{20dlanls}       & \verb|NGLBXSCTJKHFYPEMADRQfybsxjzgdntekhpamqrci/&[.]#*'{(!_||\verb|):,%@^-=;+~"}$?o>\<`VZuvwUW| \\
    \rowcolor{white}
    \textbf{8dlansd}       & \verb|8659734^;)?#`"(,.$!'%:<*]||\verb|}@-+[{~>_&=\/| \\
    \rowcolor{white}
    \textbf{12dlansd}       & \verb|4867935\?=$<||\verb|:"-!#^(+*'>,&;.@/`)%{][}~_| \\
    \rowcolor{white}
    \textbf{20dlansd}       & \verb|9358647%^".-,_(;!*]=?{+)$||\verb|~@&'[#:/}<`\>2| \\
    \\ \bottomrule
    \end{tabular}
    \caption{Dashlane Password Generation: Characters Sorted by Frequency}
    \captionsetup{aboveskip=0pt,font=it}
    \label{tab:dashlncharfreq}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lG@{}}
    \\ \midrule
    \rowcolor{white}
    \textbf{8bwall}       & \verb|9842&$3%*^6#7!5@ueDZiUkHnbTdEyfWLPSGABFjcQMrqYwmzRapCgvhxXKJIVsotN| \\
    \rowcolor{white}
    \textbf{12bwall}       & \verb|^#3@47&$628%*95!eiMxcTnFkuajdUbhDNRGgLYwfsmJXPHIWyCSvtZKrAVozqEBQp| \\
    \rowcolor{white}
    \textbf{20bwall}       & \verb|%7#9532^@46!$&8*IYBomtbJFLUPVnXdzSexagHZrwusiMkpqcWNRvQKhfDCGAjyTE| \\
    \textbf{8bwl}       & \verb|JLWRorbeGqZIwdAjnmcDyaBgHPTCfxtuXpNKikEzUsYhFVvMSQ| \\
    \textbf{12bwl}       & \verb|LwqpWREtrFkTIcuCyQnjUJZxKibgAfaDMNHXzmSdeVYPoshvGB| \\
    \textbf{20bwl}       & \verb|YywRTunfhHaxLKWcAENmMIoXbvCeZQJptrFVSigPDqkUGBdjzs| \\
    \rowcolor{white}
    \textbf{8bwld}       & \verb|68924753ricSNaCktuxGnQVJMPyDKUHpmgEqTZWwAvXRfodFILYhejbBzs| \\
    \rowcolor{white}
    \textbf{12bwld}       & \verb|95827634IUaZYgQiJnVvHoFDBftWbCzRmPXhSMpedEwTLysrcAxqGjNKku| \\
    \rowcolor{white}
    \textbf{20bwld}       & \verb|92758643EeGhznqsWUyQkcwXFLMoPuCRVNZDmHraTKSAgxpdbvftIjJBYi| \\
    \textbf{8bwls}       & \verb|&^*$@%!#uGhAIxatgfXrzdiTFNKovenBbyDVjqwcYpWLERMQJHmSCsZPkU| \\
    \textbf{12bwls}       & \verb|&$%@^!#*UFEhuAjWDBSQqTZKvGsePVkiYntbroCNMRJxmgHcawfIXdLzyp| \\
    \textbf{20bwls}       & \verb|^*&$#@%!nWUJXiChjHpzGuqkFYoebAsrdayxPBvDwMcNSmRTtVIfEQLgKZ| \\
    \rowcolor{white}
    \textbf{8bwsd}       & \verb|&93*2#47$!6@5^%8| \\
    \rowcolor{white}
    \textbf{12bwsd}       & \verb|65*7!%@2$^84#39&| \\
    \rowcolor{white}
    \textbf{20bwsd}       & \verb|7%&!654$2*^3#9@8| \\
    \\ \bottomrule
    \end{tabular}
    \caption{Bitwarden Password Generation: Characters Sorted by Frequency}
    \captionsetup{aboveskip=0pt,font=it}
    \label{tab:bitwardencharfreq}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lG@{}}
    \\ \midrule
    \rowcolor{white}
    \textbf{8passgnall}       & \verb|4617893250uTBqoGdUsgibfMwhKIvVnylmRCNazEWPJQpLXctOekHZFYxArDjS![={%*-._||\verb|);&<"}],#^`$\~'/(?@+:>| \\
    \rowcolor{white}
    \textbf{12passgnall}       & \verb|3928067415ogeNJUkABWwqxRrIzDctipbGdMfmPHyshEXuaOCQvTVLFYljSKZn-`&;$>('{\<!})||\verb|"#*]^/?[@+_~.=,:%| \\
    \rowcolor{white}
    \textbf{20passgnall}       & \verb|2475913680ZYJLoqdlDkipIWVnGaEQXUmRPMBchgNHfuAybvxTtSOCrsweFKjz\![@"(.%'||\verb|_$/:}~&<{-?,`;^#>]=+*)| \\
    \textbf{8passgnl}       & \verb|HZezDdMlKJrgwcNGkWBxLhubjqnSfYTFivUaCItpRmsAPQyVEoXO| \\
    \textbf{12passgnl}       & \verb|pdIRlDXJasZEYMuVkPbQHTmNBOAhqfyGnCxvieUFjwLWroSzgtKc| \\
    \textbf{20passgnl}       & \verb|NIPmhHdlnWjBxbpzVFAKwTCgyUQkiSurYqecvfGXEMotDaLZRsOJ| \\
    \rowcolor{white}
    \textbf{8passgnld}       & \verb|0253946871WNZRkPGVapFOTXYyeEAboujmqldMizrncwSvUtsIgLJBDKhCHxfQ| \\
    \rowcolor{white}
    \textbf{12passgnld}       & \verb|6839247105JvUSAYRomeqZVszFKQakxMpXrBTPLbfildDyNuwcOhWjngGCItEH| \\
    \rowcolor{white}
    \textbf{20passgnld}       & \verb|1546709832YGuDwpkOiylfUcHJoEWLFrvaXsbgqAzjQZBhdCMmINTPVetKRSnx| \\
    \textbf{8passgnls}       & \verb|DPdanVIFZiLmzRBJcHjwoGfEkxgOvpXUhrMWbCSqlKusAyQeTYtN$~:(%}@;{<.&`=^\/["||\verb|-']?_*)>+#!,| \\
    \textbf{12passgnls}       & \verb|ZEfKBgoWkhYiIeuUxwFqcvXANGTjHSpldntVbayJsCzRrOmPDLQM*^(>-['~{":_],<?+=\!%||\verb|@.)`/}$#;&| \\
    \textbf{20passgnls}       & \verb|qbSeLXKANmwjZkRcVapPzYfDgOvTtnIGUdliJsFyWBHMoQhExuCr@,\$}/!`:]||\verb|({[)'.#?*&><;~+_"-=%^| \\
    \rowcolor{white}
    \textbf{8passgnsd}       & \verb|1924305786||\verb|[^}(/`.~$#<>)_{-:,\@"'&!=]*?;+%| \\
    \rowcolor{white}
    \textbf{12passgnsd}       & \verb|9630571842'~^*,>-\!<`#}([?=||\verb|]@"/):+{;$_%.&| \\
    \rowcolor{white}
    \textbf{20passgnsd}       & \verb|2360957841'!.;&%~/#[_>}+-<*:){@="?`(\$||\verb|,]^| \\
    \\ \bottomrule
    \end{tabular}
    \caption{Password Generator Password Generation: Characters Sorted by Frequency}
    \captionsetup{aboveskip=0pt,font=it}
    \label{tab:passgencharfreq}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lggG@{}}
           \rowcolor{white} 
           & \textbf{mean (\%)}
           & \textbf{std (\%)}
           & \textbf{sorted outliers}
    \\ \midrule
    \rowcolor{white}
    \textbf{20roboall} & 1.59 & 0.24 & \verb|%#@!^$8462735zZ9| \\
    \textbf{20robol} & 2.08 & 0.03 & \verb|Z| \\
    \rowcolor{white}
    \textbf{20robold} & 1.79 & 0.17 & \verb|6532874Z9| \\
    \textbf{20robols} & 1.82 & 0.2 & \verb|%@$^#!Zz| \\
    \rowcolor{white}
    \textbf{20robosd} & 7.14 & 0.21 & \verb|9| \\
    \textbf{20lpassall} & 1.43 & 0.16 & \verb|%$&!#@*^7605428139| \\
    \rowcolor{white}
    \textbf{20lpassld} & 1.61 & 0.07 & \verb|451| \\
    \textbf{20lpassls} & 1.67 & 0.15 & \verb|%&*@#$!^| \\
    \rowcolor{white}
    \textbf{20bwall} & 1.52 & 0.18 & \verb|%7#9532^@46!$&8*| \\
    \textbf{20bwld} & 1.72 & 0.15 & \verb|92758643| \\
    \rowcolor{white}
    \textbf{20bwls} & 1.72 & 0.15 & \verb|^*&$#@%!| \\
    \textbf{20dlanall} & 1.12 & 0.26 & \verb|ZVvW2Uuw\<>57`63948o| \\
    \rowcolor{white}
    \textbf{20dlanl} & 2.04 & 0.47 & \verb|UZWvwVuoMXHQEDNTFLCGJBKYPRSAbjhtpqz| \\
    \textbf{20dlanld} & 1.75 & 0.41 & \verb|v2wUWZVuo4573689| \\
    \rowcolor{white}
    \textbf{20dlanls} & 1.23 & 0.25 & \verb|WUwvuZV`<\>oNGLBXSCTJKHFYPEMADR| \\
    \textbf{20dlansd} & 2.5 & 0.45 & \verb|2>\`<9358647| \\
    \rowcolor{white}
    \textbf{20passgnall} & 1.06 & 0.1 & \verb|2475913680| \\
    \textbf{20passgnld} & 1.61 & 0.11 & \verb|1546709832| \\
    \rowcolor{white}
    \textbf{20passgnsd} & 2.38 & 0.15 & \verb|2360957841| \\
    \\ \bottomrule
    \end{tabular}
    \caption{Length 20 Character Frequency Outliers}
    \captionsetup{aboveskip=0pt,font=it}
    \caption*{\\Values not shown had no outliers}
    \label{tab:freqoutliers20}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lggG@{}}
           \rowcolor{white} 
           & \textbf{mean (\%)}
           & \textbf{std (\%)}
           & \textbf{sorted outliers}
    \\ \midrule
    \rowcolor{white}
    \textbf{12roboall} & 1.59 & 0.39 & \verb|$%#^!@2637548Zz9ruyfxmpwgciaqvjkshneobtdKTPVLAUMNDRJYWXCEQSFGHB| \\
    \textbf{12robol} & 2.08 & 0.05 & \verb|Z| \\
    \rowcolor{white}
    \textbf{12robold} & 1.79 & 0.29 & \verb|68532479Z| \\
    \textbf{12robols} & 1.82 & 0.33 & \verb|$^%#@!zZ| \\
    \rowcolor{white}
    \textbf{12robosd} & 7.14 & 0.35 & \verb|9| \\
    \textbf{12lpassall} & 1.43 & 0.27 & \verb|*@$&!#%^7893024156| \\
    \rowcolor{white}
    \textbf{12lpassld} & 1.61 & 0.12 & \verb|5683419027| \\
    \textbf{12lpassls} & 1.67 & 0.24 & \verb|!@#^%&*$| \\
    \rowcolor{white}
    \textbf{12lpasssd} & 5.56 & 0.52 & \verb|^#!*@$&%| \\
    \textbf{12bwall} & 1.52 & 0.3 & \verb|^#3@47&$628%*95!pQBEqzoVArKZtvSCyWIHPXJmsfwYLgGRNDhbUdjaukFnTcxMie| \\
    \rowcolor{white}
    \textbf{12bwld} & 1.72 & 0.24 & \verb|95827634| \\
    \textbf{12bwls} & 1.72 & 0.24 & \verb|&$%@^!#*| \\
    \rowcolor{white}
    \textbf{12onepsall} & 1.3 & 0.12 & \verb|9537168402| \\
    \textbf{12onepsld} & 1.72 & 0.09 & \verb|1304286957| \\
    \rowcolor{white}
    \textbf{12dlanall} & 1.23 & 0.25 & \verb|3498576&@%[)_>};:|\verb|`+'^*~.]=\("?,-<!{#$/| \\
    \textbf{12dlanld} & 2.04 & 0.28 & \verb|6859743| \\
    \rowcolor{white}
    \textbf{12dlansd} & 2.56 & 0.36 & \verb|4867935| \\
    \textbf{12passgnall} & 1.06 & 0.17 & \verb|3928067415| \\
    \rowcolor{white}
    \textbf{12passgnld} & 1.61 & 0.19 & \verb|6839247105| \\
    \textbf{12passgnsd} & 2.38 & 0.24 & \verb|9630571842| \\
    \\ \bottomrule
    \end{tabular}
    \caption{Length 12 Character Frequency Outliers}
    \captionsetup{aboveskip=0pt,font=it}
    \caption*{\\Values not shown had no outliers}
    \label{tab:freqoutliers12}
    \end{center}
\end{table*}

\begin{table*}
    \begin{center}
    \begin{tabular}{@{}lggG@{}}
           \rowcolor{white} 
           & \textbf{mean (\%)}
           & \textbf{std (\%)}
           & \textbf{sorted outliers}
    \\ \midrule
    \rowcolor{white}
    \textbf{8roboall} & 1.59 & 0.59 & \verb|%!^@$#46275839zZjcrwdxiyhubtpvfkoensagmqWYVQLKBREMGSTCAXUJDFHPN| \\
    \textbf{8robol} & 2.08 & 0.08 & \verb|Z| \\
    \rowcolor{white}
    \textbf{8robold} & 1.79 & 0.43 & \verb|57823469Z| \\
    \textbf{8robols} & 1.82 & 0.5 & \verb|%@^$#!Zz| \\
    \rowcolor{white}
    \textbf{8robosd} & 7.14 & 0.52 & \verb|9| \\
    \textbf{8lpassall} & 1.43 & 0.4 & \verb|$*!@^#&%9460832175| \\
    \rowcolor{white}
    \textbf{8lpassld} & 1.61 & 0.18 & \verb|5269480173| \\
    \textbf{8lpassls} & 1.67 & 0.37 & \verb|%&$*^#@!| \\
    \rowcolor{white}
    \textbf{8lpasssd} & 5.56 & 0.78 & \verb|@!#^%*$&5916820347| \\
    \textbf{8bwall} & 1.52 & 0.46 & \verb|9842&$3%*^6#7!5@NtosVIJKXxhvgCpaRzmwYqrMQcjFBAGSPLWyfEdTbnHkUiZDeu| \\
    \rowcolor{white}
    \textbf{8bwld} & 1.72 & 0.37 & \verb|68924753| \\
    \textbf{8bwls} & 1.72 & 0.37 & \verb|&^*$@%!#| \\
    \rowcolor{white}
    \textbf{8onepsall} & 1.3 & 0.25 & \verb|1486075923dxnyLHRqemJBNtirYuoGvZAEPgXhKzVTbFaDkfsWQjUcCpwM| \\
    \textbf{8onepsld} & 1.72 & 0.22 & \verb|4095683721| \\
    \rowcolor{white}
    \textbf{8dlanall} & 1.23 & 0.37 & \verb|7849536^\}+-?&:#'@`>)%,/<~[;!]{|\verb|_=*."$(| \\
    \textbf{8dlanld} & 2.04 & 0.42 & \verb|9457368ez| \\
    \rowcolor{white}
    \textbf{8dlansd} & 2.56 & 0.54 & \verb|8659734/\=&| \\
    \textbf{8passgnall} & 1.06 & 0.25 & \verb|4617893250>:+@?(/'~\$`^#,]}"<&;)|\verb|_.-*%{=[!| \\
    \textbf{8passgnld} & 1.61 & 0.28 & \verb|0253946871| \\
    \textbf{8passgnsd} & 2.38 & 0.37 & \verb|1924305786| \\
    \\ \bottomrule
    \end{tabular}
    \caption{Length 8 Character Frequency Outliers}
    \captionsetup{aboveskip=0pt,font=it}
    \caption*{\\Values not shown had no outliers}
    \label{tab:freqoutliers8}
    \end{center}
\end{table*}
